Bounded-Regret MPC via Perturbation Analysis: Prediction Error, Constraints, and Nonlinearity

We study Model Predictive Control (MPC) and propose a general analysis pipeline to bound its dynamic regret. The pipeline first requires deriving a perturbation bound for a finite-time optimal control problem. Then, the perturbation bound is used to bound the per-step error of MPC, which leads to a bound on the dynamic regret. Thus, our pipeline reduces the study of MPC to the well-studied problem of perturbation analysis, enabling the derivation of regret bounds of MPC under a variety of settings. To demonstrate the power of our pipeline, we use it to generalize existing regret bounds on MPC in linear time-varying (LTV) systems to incorporate prediction errors on costs, dynamics, and disturbances. Further, our pipeline leads to regret bounds on MPC in systems with nonlinear dynamics and constraints.

==> 5-lower_bound.tex <==
The constrained LTV system is fundamentally different with the unconstrained LTV system considered in \cite{lin2021perturbation}. Even in the simplest case, the exponentially decaying perturbation bound does not hold.

\begin{theorem}\label{thm:exp-decay-impossible}
Consider the specific instance of \eqref{equ:auxiliary_control_problem} where $n = m = 1$. Suppose
\[A_t = B_t = 1, \mathcal{X}_t = \{x\mid -1 \leq x \leq 1\}, \mathcal{U}_t = \{u\mid -1 \leq u \leq 1\}, Q_t = 1, R_t = 0, \delta_t = 0\]
holds for all $t$. Let $w_t = 1$ if $t$ is odd, and $w_t = -1$ if $t$ is even. For any $H$ is even, we have
\[\abs{\psi_{0}^H\left(0, -\frac{1}{2}, w_{1:H-1}, 0\right)_{x_h} - \psi_{0}^H\left(0, -\frac{1}{2} + \frac{1}{2(H - 1)}, w_{1:H-1}, 0\right)_{x_h}} = \frac{1}{2(H-1)}\]
holds for any $h \in \{1, \ldots, H\}$. For any $H$ is odd, we have
\[\abs{\psi_{0}^H\left(0, \frac{1}{2}, w_{1:H-1}, 0\right)_{x_h} - \psi_{0}^H\left(0, \frac{1}{2} + \frac{1}{2H}, w_{1:H-1}, 0\right)_{x_h}} = \frac{1}{2H}\]
holds for any $h \in \{1, \ldots, H\}$.
\end{theorem}

\textbf{Remark:} \Cref{thm:exp-decay-impossible} implies that exponentially decaying perturbation bound cannot hold even for a simple class of constrained control problems. Further, the decay rate in the perturbation bound cannot be better than $\Omega(1)$.

\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{Figures/perturbation_counterexample.png}
    \caption{Illustration of the perturbation lower bound in \Cref{thm:exp-decay-impossible} for $H = 8$. The blue/red curve plots the original/perturbed optimal state trajectory for the instance described in \Cref{thm:exp-decay-impossible}.}
    \label{fig:perturbation_lower_bound}
\end{figure}

\begin{proof}[Proof of \Cref{thm:exp-decay-impossible}]
It is straightforward to verify that when $H$ is even,
\begin{align*}
    \psi_{0}^H\left(0, -\frac{1}{2}, w_{1:H-1}, 0\right)_{x_{h}} &= \begin{cases}
        \frac{1}{2}, \text{ if }h\equiv 1 (\text{mod }2),\\
        -\frac{1}{2}, \text{ otherwise,}
    \end{cases}\\
    \psi_{0}^H\left(0, -\frac{1}{2}+\frac{1}{2(H-1)}, w_{1:H-1}, 0\right)_{x_h} &= \begin{cases}
        \frac{1}{2} + \frac{1}{2(H-1)}, \text{ if }h\equiv 1 (\text{mod }2),\\
        -\frac{1}{2} + \frac{1}{2(H-1)}, \text{ otherwise,}
    \end{cases}
\end{align*}
for all $h \in \{1, \ldots, H\}$. We also see that when $H$ is odd,
\begin{align*}
    \psi_{0}^H\left(0, \frac{1}{2}, w_{1:H-1}, 0\right)_{x_{h}} &= \begin{cases}
        \frac{1}{2}, \text{ if }h\equiv 1 (\text{mod }2),\\
        -\frac{1}{2}, \text{ otherwise,}
    \end{cases}\\
    \psi_{0}^H\left(0, \frac{1}{2}+\frac{1}{2H}, w_{1:H-1}, 0\right)_{x_h} &= \begin{cases}
        \frac{1}{2} + \frac{1}{2H}, \text{ if }h\equiv 1 (\text{mod }2),\\
        -\frac{1}{2} + \frac{1}{2H}, \text{ otherwise,}
    \end{cases}
\end{align*}
for all $h \in \{1, \ldots, H\}$.
\end{proof}

Recall that in \cite{lin2021perturbation}, the authors showed that MPC can achieve a competitive ratio of $1 + O(\rho^k)$ when $\mathcal{X}_t = \mathbb{R}^n, \mathcal{U}_t = \mathbb{R}^m$. Their result heavily relies on a exponentially decaying perturbation bound on the optimal solution. Indeed, the perturbation bound is critical for the online controller's performance because \yiheng{explain the reason...}
Given that the perturbation bound cannot achieve better than $1/H$ decay rate, a natural question to ask is whether it implies a corresponding lower bound on the competitive ratio for any online controllers. The following corollary answers this question:

\begin{theorem}\label{thm:lower-bound-online-controller}
Consider a special class of the online control problem \eqref{equ:online_control_problem} where
\[A_t = B_t = 1, \mathcal{X}_t = \{x\mid -1 \leq x \leq 1\}, \mathcal{U}_t = \{u\mid -1 \leq u \leq 1\}, Q_t = 1, R_t = 0\]
for all time $t$. Suppose an online controller $ALG$ has access to $k$ steps of exact predictions of $(w_t, \delta_t)$. For arbitrary prediction horizon $k$, there exists a problem instance that satisfies Assumption \ref{assump:controllability} and Assumption \ref{assump:uniform-controllability} where
\[\frac{\cost(ALG)}{\cost(OPT)} \geq 1 + \Omega\left(\frac{1}{k^2}\right).\]
\end{theorem}

\begin{proof}[Proof of \Cref{thm:lower-bound-online-controller}]
Consider the same problem instance as constructed in \Cref{thm:exp-decay-impossible} where the initial state is $0$ and
\begin{equation*}
    w_t = \begin{cases}
    1 & \text{ if } t \equiv 1(\text{mod }2),\\
    0 & \text{ otherwise.}
    \end{cases}
\end{equation*}

After the online controller picks the $u_0$ and the system evolves to $x_1$, the adversary decides $w_{k+1}$ and $w_{k+2}$ based on $x_1$:
\begin{enumerate}
    \item If $k$ is odd and $x_1 \geq \frac{1}{2} + \frac{1}{4(H - 1)}$, the adversary picks $w_{k+1} = -1, w_{k+2} = 0$;
    \item If $k$ is odd and 
\end{enumerate}

If $k$ is odd, the adversary picks
\begin{align*}
    w_{k+1} = \begin{cases}
        -1 & \text{ if } x_1 \geq \frac{1}{2} + \frac{1}{4(H - 1)},\\
        0 & \text{ otherwise.}
    \end{cases}
\end{align*}
By picking the terminal state in this way, we see that: If $x_1 \geq \frac{1}{2} + \frac{1}{4(H - 1)}$,
\end{proof}

==> Figures/pipeline.tex <==
\begin{tikzpicture}
    \draw[draw=orange, line width=3.0pt, ->, >={Stealth}] (10pt, 0pt) -- (10pt, -25pt) -- (35pt, -25pt);
    \node[above=1pt] at (20pt, -25pt) {\eqref{equ:perturbation-bound-fix-initial}};
    \begin{scope}[xshift=35pt, yshift=-10pt]
        \draw[draw=black, line width=1.0pt] (0pt, 0pt) rectangle (60pt, -30pt);
        \node at (30pt, -9pt) {initial bound};
        \node at (30pt, -21pt) {on $e_t$ \eqref{equ:pipeline-initial-bound-e-t}};
    \end{scope}
    
    \draw[draw=DarkBlue, line width=3.0pt, ->, >={Stealth}] (5pt, 0pt) -- (5pt, -65pt) -- (35pt, -65pt);
    \node[above=1pt] at (20pt, -65pt) {\eqref{equ:perturbation-bound-fix-parameters}};
    \begin{scope}[xshift=35pt, yshift=-50pt]
        \draw[draw=black, line width=1.0pt] (0pt, 0pt) rectangle (60pt, -30pt);
        \node at (30pt, -9pt) {initial bound};
        \node at (30pt, -21pt) {on $\norm{x_t}$ \eqref{equ:pipeline-initial-bound-x-t}};
    \end{scope}
    
    \begin{scope}[xshift=105pt, yshift=-45pt]
        %\draw[draw=lightgray, line width=3.0pt, dotted, ->, >={Stealth}] (-5pt, 0pt) -- (50pt, 0pt);
        \foreach \x in {0,1,2,3,4,5}
          { \fill[fill=lightgray] (6*\x pt-5pt, 0pt) circle (1.5pt); }
          \draw[draw=lightgray, line width=3.0pt, ->, >={Stealth}] (30pt, 0pt) -- (50pt, 0pt);
        
        \node at (18pt, 8pt) {alternating};
        \node at (18pt, -7pt) {bound};
        \node at (18pt, -17pt) {refinement};
    \end{scope}
    
    \begin{scope}[xshift=155pt, yshift=-10pt]
        \draw[draw=black, line width=1.0pt] (0pt, 0pt) rectangle (40pt, -30pt);
        \node at (20pt, -9pt) {bound};
        \node at (20pt, -21pt) {on $e_t$};
    \end{scope}
    
    \begin{scope}[xshift=155pt, yshift=-50pt]
        \draw[draw=black, line width=1.0pt] (0pt, 0pt) rectangle (40pt, -30pt);
        \node at (20pt, -9pt) {stability};
        \node at (20pt, -21pt) {of $\norm{x_t}$};
    \end{scope}
    
    \draw[draw=black, line width=1.0pt, dashed] (30pt, -5pt) rectangle (200pt, -85pt);
    \node[below=1pt] at (115pt, -85pt) {\textit{Step 2.} obtain refined bounds on $e_t$};
    
    \draw[draw=DarkBlue, line width=3.0pt, ->, >={Stealth}] (290pt, 0pt) -- (290pt, -37pt);
    \node[left=1pt] at (290pt, -12.5pt) {\eqref{equ:perturbation-bound-fix-parameters}};
    \begin{scope}[xshift=265pt, yshift=-45pt]
        \fill[fill=pink] (0pt, 8pt) -- (45pt, 8pt) -- (45pt, 15pt) -- (55pt, 0pt) -- (45pt, -15pt) -- (45pt, -8pt) -- (0pt, -8pt) -- cycle;
        \node at (27pt, 0pt) {\Cref{thm:per-step-error-to-performance-guarantee}};
    \end{scope}
    
    \draw[draw=lightgray, line width=3.0pt, ->, >={Stealth}] (195pt, -25pt) -- (205pt, -25pt) -- (205pt, -45pt) -- (225pt, -45pt);
    \begin{scope}[xshift=225pt, yshift=-25pt]
        \draw[draw=black, line width=1.0pt] (0pt, 0pt) rectangle (40pt, -40pt);
        \node at (20pt, -14pt) {bound on};
        \node at (20pt, -26pt) {$\sum_{t} e_t^2$};
    \end{scope}
    
    \begin{scope}[xshift=320pt, yshift=-25pt]
        \draw[draw=black, line width=1.0pt] (0pt, 0pt) rectangle (50pt, -40pt);
        \node at (25pt, -11pt) {dynamical};
        \node at (25pt, -21pt) {regret};
        \node at (25pt, -30pt) {bound};
    \end{scope}
    
    \draw[draw=black, line width=1.0pt, dashed] (220pt, -20pt) rectangle (375pt, -70pt);
    \node[below=1pt] at (300pt, -70pt) {\textit{Step 3.} obtain dynamical regret bound};
    
    \draw[draw=black, line width=1.0pt] (0pt, 16pt) rectangle (380pt, 0pt);
    \node at (190pt, 8pt) {\textit{Step 1.} obtain general perturbation bounds \eqref{equ:perturbation-bound-fix-initial} \& \eqref{equ:perturbation-bound-fix-parameters}};
\end{tikzpicture}

==> LTV_perturbation_bounds.tex <==
We will follow the two-time-scale scheme illustrated in Figure \ref{fig:LTV-reduction-to-SOCO} to reduce the constrained LTV optimization problem to a constrained SOCO problem on a larger time-scale. The new switching cost will be defined as
\[\hat{c}_\tau\left(\hat{x}_\tau, \hat{x}_{\tau-1}, \zeta_{\tau-1}^c\right) \coloneqq \iota_{(\tau-1) d}^{\tau d}\left(y_{(\tau - 1) d}, y_{\tau d}, w_{(\tau - 1)d+1:\tau d-1}, \delta_{(\tau - 1)d:\tau d-1}\right),\]
where $\hat{x}_\tau = y_{\tau d}, \hat{x}_{\tau - 1} = y_{(\tau - 1)d}$, and $\zeta_{\tau-1}^c = \left(w_{(\tau - 1)d+1:\tau d-1}, \delta_{(\tau - 1)d:\tau d-1}\right)$. We will show the new switching cost is convex and smooth by studying the property of $\psi_{t_1}^{t_2}$. To simplify the notation, we will use $\upsilon_{t_1}^{t_2}$ to denote the parameter tuple $\left(y_{t_1}, y_{t_2}, w_{t_1+1:t_2-1}, \delta_{t_1:t_2-1}\right)$.

\begin{figure}
    \centering
    \includegraphics[width=.7\textwidth]{Figures/SOCO_2scale_reduction.drawio.png}
    \caption{Illustration of the reduction from constrained LTV system to constrained SOCO.}
    \label{fig:LTV-reduction-to-SOCO}
\end{figure}

\begin{lemma}\label{lemma:switching-cost-opt-sol}
When $t_1$ and $t_2$ are fixed and satisfies $t_2 \in [t_1 + d, t_1 + 2d)$, $\psi_{t_1}^{t_2}$ is a well-defined function from $\mathcal{X}_{t_1} \times \mathcal{X}_{t_2} \times (\mathbb{R}^{n})^{t_2 - t_1 - 1} \times \left(\mathbb{R}^{m}\right)^{t_2 - t_1}$ to $(\mathbb{R}^{n})^{t_2 - t_1 - 1} \times \left(\mathbb{R}^{m}\right)^{t_2 - t_1}$. Further, $\psi_{t_1}^{t_2}$ is continuous and piece-wise affine in its parameter $\upsilon_{t_1}^{t_2}$, and satisfies
\[\norm{\psi_{t_1}^{t_2}\left(\upsilon_{t_1}^{t_2}\right) - \psi_{t_1}^{t_2}\left((\upsilon_{t_1}^{t_2})'\right)} \leq L_2 \norm{\upsilon_{t_1}^{t_2} - (\upsilon_{t_1}^{t_2})'}\]
where
\[L_2 = L_2()\]
\end{lemma}
\begin{proof}[Proof of \Cref{lemma:switching-cost-opt-sol}]
\input{Proofs/switching-cost-opt-sol}
\end{proof}

==> Proofs/Lipschitz-global-opt-sol.tex <==
To simplify the notation, we will use a single vector $\xi$ to denote the original parameters tuple $\left(\hat{y}_0, \hat{y}_\horizonvar, \zeta_{1:H-1}^f, \zeta_{0:H-1}^c\right)$, and use $\xi'$ to denote the perturbed parameters tuple $\left(\hat{y}_0', \hat{y}_\horizonvar', (\zeta_{1:H-1}^f)', (\zeta_{0:H-1}^c)'\right)$. We also denote the objective function as
\begin{align}\label{thm:Lipschitz-global-opt-sol:e0}
    \hat{F}(\hat{x}_{1:H-1}, \xi) \coloneqq \sum_{\tau=1}^{\horizonvar-1} \hat{f}_\tau\left(\hat{x}_\tau, \zeta_\tau^f\right) + \sum_{\tau=1}^{\horizonvar} \hat{c}_\tau\left(\hat{x}_\tau, \hat{x}_{\tau - 1}, \zeta_{\tau-1}^c\right).
\end{align}
Since the objective function is $\hat{\mu}_f$-strongly convex for any fixed set of parameter, we see that
\begin{subequations}\label{thm:Lipschitz-global-opt-sol:e1}
\begin{align}
    \hat{F}\left(\hat{\psi}(\xi'), \xi\right) - \hat{F}\left(\hat{\psi}(\xi), \xi\right) \geq{}& \frac{\hat{\mu}_f}{2}\norm{\hat{\psi}(\xi') - \hat{\psi}(\xi)}^2,\label{thm:Lipschitz-global-opt-sol:e1:s1}\\
    \hat{F}\left(\hat{\psi}(\xi), \xi'\right) - \hat{F}\left(\hat{\psi}(\xi'), \xi'\right) \geq{}& \frac{\hat{\mu}_f}{2}\norm{\hat{\psi}(\xi') - \hat{\psi}(\xi)}^2,\label{thm:Lipschitz-global-opt-sol:e1:s2}
\end{align}
\end{subequations}
where we used the fact that $\hat{\psi}(\xi)$ is the minimizer of the $\hat{\mu}_f$-strongly convex function $\hat{F}(\cdot, \xi)$ in the convex domain $\prod_{\tau=1}^{H-1}\hat{\mathcal{X}}_\tau$ in \eqref{thm:Lipschitz-global-opt-sol:e1:s1}; similarly, in \eqref{thm:Lipschitz-global-opt-sol:e1:s2}, $\hat{\psi}(\xi')$ is the minimizer of the $\hat{\mu}_f$-strongly convex function $\hat{F}(\cdot, \xi')$ in the same domain.

Note that when $\hat{x}_{1:H-1}$ are fixed, $\hat{F}(\hat{x}_{1:H-1}, \cdot)$ is a $\hat{\ell} \coloneqq \max(\hat{\ell}_f, \hat{\ell}_c)$-smooth function. Thus we see that
\begin{subequations}\label{thm:Lipschitz-global-opt-sol:e2}
\begin{align}
    \hat{F}\left(\hat{\psi}(\xi'), \xi\right) - \hat{F}\left(\hat{\psi}(\xi'), \xi'\right) \leq{}& \langle \nabla_2 \hat{F}\left(\hat{\psi}(\xi'), \xi'\right), \xi - \xi'\rangle + \frac{\hat{\ell}}{2}\norm{\xi - \xi'}^2\label{thm:Lipschitz-global-opt-sol:e2:s1}\\
    \hat{F}\left(\hat{\psi}(\xi), \xi'\right) - \hat{F}\left(\hat{\psi}(\xi), \xi\right) \leq{}& \langle \nabla_2 \hat{F}\left(\hat{\psi}(\xi), \xi\right), \xi' - \xi\rangle + \frac{\hat{\ell}}{2}\norm{\xi - \xi'}^2.\label{thm:Lipschitz-global-opt-sol:e2:s2}
\end{align}
\end{subequations}
Subtracting \eqref{thm:Lipschitz-global-opt-sol:e1:s1} and \eqref{thm:Lipschitz-global-opt-sol:e1:s2} from the sum of \eqref{thm:Lipschitz-global-opt-sol:e2:s1} and \eqref{thm:Lipschitz-global-opt-sol:e2:s2} gives that
\begin{align*}
    &\hat{\mu}_f \norm{\hat{\psi}(\xi') - \hat{\psi}(\xi)}^2\\
    \leq{}& \langle \nabla_2 \hat{F}\left(\hat{\psi}(\xi'), \xi'\right) - \nabla_2 \hat{F}\left(\hat{\psi}(\xi), \xi\right), \xi - \xi'\rangle + \hat{\ell} \norm{\xi - \xi'}^2.
\end{align*}
The right hand side of the above inequality can be further bounded by
\begin{align*}
    RHS \leq{}& \norm{\nabla_2 \hat{F}\left(\hat{\psi}(\xi'), \xi'\right) - \nabla_2 \hat{F}\left(\hat{\psi}(\xi), \xi\right)}\cdot \norm{\xi - \xi'} + \hat{\ell} \norm{\xi - \xi'}^2\\
    \leq{}& (\hat{\ell}_f + 2 \hat{\ell}_c)\left(\norm{\hat{\psi}(\xi') - \hat{\psi}(\xi)} + \norm{\xi - \xi'}\right)\cdot \norm{\xi - \xi'} + \hat{\ell} \norm{\xi - \xi'}^2,
\end{align*}
where we used the fact that $\hat{F}$ is $(\ell_f + 2\ell_c)$-smooth in all of its parameters. Thus we see that
\[\norm{\hat{\psi}(\xi') - \hat{\psi}(\xi)} \leq \left(\frac{\hat{\ell}_f + 2\hat{\ell}_c + \sqrt{(\hat{\ell}_f + 2\hat{\ell}_c)^2 + 4(\hat{\ell}_f + 2\hat{\ell}_c + \hat{\ell})}}{2\hat{\mu}_f}\right)\cdot \norm{\xi - \xi'}.\]

==> Proofs/SOCO-sensitivity.tex <==
With some slight abuse of notation, we define 
\[\zeta^f(\tau) \coloneqq \left((\zeta_1^f)', \ldots, (\zeta_{\tau-1}^f)', \zeta_\tau^f, \ldots, \zeta_{H-1}^f\right), \zeta^c(\tau) \coloneqq \left((\zeta_0^c)', \ldots, (\zeta_{\tau-1}^c)', \zeta_\tau^c, \ldots, \zeta_{H-1}^c\right)\]
with the convention that $\zeta^f(1) = \zeta_{1:H-1}^f, \zeta^c(0) = \zeta_{0:H-1}^c$ and $\zeta^f(H) = (\zeta_{1:H-1}^f)', \zeta^c(H) = (\zeta_{0:H-1}^c)'$. To connect with \Cref{thm:well-cond-grad-descent-with-constraints}, we let $\hat{F}$ denote the objective function as \eqref{thm:Lipschitz-global-opt-sol:e0}, and let $\hat{\mathcal{Q}}\coloneqq \prod_{\tau=1}^{H-1} \hat{\mathcal{X}}_\tau$. Vector $z$ in \Cref{thm:well-cond-grad-descent-with-constraints} will denote the solution vector $\hat{x}_{1:H-1}$ in \Cref{thm:SOCO-sensitivity}.

We first show that for any $\tau \in \{0, \ldots, H-1\}$,
\begin{align}\label{thm:SOCO-sensitivity-e1}
    &\norm{\hat{\psi}\left(\hat{y}_0', \hat{y}_H, \zeta^f(\tau + 1), \zeta^c(\tau)\right)_h - \hat{\psi}\left(\hat{y}_0', \hat{y}_H, \zeta^f(\tau + 1), \zeta^c(\tau + 1)\right)_h}\nonumber\\
    \leq{}& C_0 \lambda_0^{\abs{h - \tau}} \norm{\zeta_\tau^c - (\zeta_\tau^c)'}.
\end{align}
To show \eqref{thm:SOCO-sensitivity-e1}, we run the iterative gradient-based update rule in \eqref{thm:well-cond-grad-descent-with-constraints:update-rule} to solve the optimization problem \eqref{equ:large-scale-SOCO} with parameters $\xi \coloneqq \left(\hat{y}_0', \hat{y}_H, \zeta^f(\tau + 1), \zeta^c(\tau + 1)\right)$ from the initial point $z(0) \coloneqq \hat{\psi}\left(\hat{y}_0', \hat{y}_H, \zeta^f(\tau + 1), \zeta^c(\tau)\right)$. Here, $z^* = \hat{\psi}\left(\hat{y}_0', \hat{y}_H, \zeta^f(\tau + 1), \zeta^c(\tau + 1)\right)$

Note that the global update rule in \eqref{thm:well-cond-grad-descent-with-constraints:update-rule}, and \eqref{thm:well-cond-grad-descent-with-constraints:gradient-map:s1}, \eqref{thm:well-cond-grad-descent-with-constraints:gradient-map:s2} can be written equivalently for each $i \in \{1, \ldots, H-1\}$ as
\[z(s+1)_i = z(s)_i - \frac{1}{\hat{\ell}_F} g_{\hat{\mathcal{Q}}}\left(z(s); \hat{\ell}_F\right)_i,\]
and
\begin{align*}
    z_{\hat{\mathcal{Q}}}\left(\bar{x}_{1:H-1}; \gamma\right)_i ={}& \argmin_{x_i \in \hat{\mathcal{X}}_i}\left(\hat{f}_i\left(\bar{x}_i, \zeta^f(\tau+1)_i\right) + \langle \nabla_i\hat{F}(\bar{x}_{1:H-1}, \xi), x_i - \bar{x}_i\rangle + \frac{\gamma}{2}\norm{x_i - \bar{x}_i}^2\right),\\
    g_{\hat{\mathcal{Q}}}(\bar{x}_{1:H-1}; \gamma)_i ={}& \gamma\left(\bar{x}_i - z_{\hat{\mathcal{Q}}}(\bar{x}_{1:H-1}; \gamma)_i\right),
\end{align*}
where
\begin{align*}
    \nabla_i\hat{F}(\bar{x}_{1:H-1}, \xi) ={}& \nabla_1\hat{c}_i(\bar{x}_i, \bar{x}_{i-1}, \zeta^c(\tau+1)_{i-1}) + \nabla_1 \hat{f}_i(\bar{x}_i, \zeta^f(\tau+1)_i)\\
    &+ \nabla_2\hat{c}_{i+1}(\bar{x}_{i+1}, \bar{x}_{i}, \zeta^c(\tau+1)_{i}).
\end{align*}
Therefore, $z(s+1)_i$ is decided by $z(s)_{i-1}, z(s)_i, z(s)_{i+1}$ and $\zeta^c(\tau+1)_{i-1}, \zeta^f(\tau+1)_i, \zeta^c(\tau+1)_{i}$. If we have
\[z(s)_{i-1:i+1} = z(0)_{i-1:i+1} \text{ and }\zeta^c(\tau+1)_{i-1:i} = \zeta^c(\tau)_{i-1:i},\]
we also have $z(s+1)_i = z(s)_i = z(0)_i$. Hence, one can use induction to show $z(s)_i = z(0)_i$ holds if $s < \abs{\tau - i}$. Therefore, when $\abs{h - \tau} \geq 1$, we see that
\begin{subequations}\label{thm:SOCO-sensitivity-e2}
\begin{align}
    &\norm{\hat{\psi}\left(\hat{y}_0', \hat{y}_H, \zeta^f(\tau + 1), \zeta^c(\tau)\right)_h - \hat{\psi}\left(\hat{y}_0', \hat{y}_H, \zeta^f(\tau + 1), \zeta^c(\tau + 1)\right)_h}\nonumber\\
    \leq{}& \norm{z(\abs{h - \tau} - 1) - z^*}\label{thm:SOCO-sensitivity-e2:s1}\\
    \leq{}& \left(1 - \frac{\hat{\mu}_c}{\hat{\ell}_f + 2\hat{\ell}_c}\right)^{\frac{\abs{h - \tau} - 1}{2}} \cdot \norm{z(0) - z^*}\label{thm:SOCO-sensitivity-e2:s2}\\
    ={}& \left(1 - \frac{\hat{\mu}_c}{\hat{\ell}_f + 2\hat{\ell}_c}\right)^{\frac{\abs{h - \tau} - 1}{2}} \cdot \norm{\hat{\psi}\left(\hat{y}_0', \hat{y}_H, \zeta^f(\tau + 1), \zeta^c(\tau)\right) - \hat{\psi}\left(\hat{y}_0', \hat{y}_H, \zeta^f(\tau + 1), \zeta^c(\tau + 1)\right)} \nonumber\\
    \leq{}& L_1 \left(1 - \frac{\hat{\mu}_c}{\hat{\ell}_f + 2\hat{\ell}_c}\right)^{\frac{\abs{h - \tau} - 1}{2}} \cdot \norm{\zeta_\tau^c - (\zeta_\tau^c)'},\label{thm:SOCO-sensitivity-e2:s3}
\end{align}
\end{subequations}
where in \eqref{thm:SOCO-sensitivity-e2:s1}, we used the fact that $z(\abs{h - \tau} - 1)_h = z(0)_h$ because the $h$ th entry in the solution vector has not been updated until iteration $\abs{h - \tau} - 1$ since iteration $0$; we used \Cref{thm:well-cond-grad-descent-with-constraints} in \eqref{thm:SOCO-sensitivity-e2:s2}; we used \Cref{lemma:Lipschitzness-of-global-optimal-solution} in \eqref{thm:SOCO-sensitivity-e2:s3}. Note that \eqref{thm:SOCO-sensitivity-e1} also holds when $\abs{h - \tau} = 0$ by \Cref{lemma:Lipschitzness-of-global-optimal-solution}.

Using the same technique as the proof of \eqref{thm:SOCO-sensitivity-e1}, we can show that
\begin{align}\label{thm:SOCO-sensitivity-e3}
    \norm{\hat{\psi}\left(\hat{y}_0', \hat{y}_H, \zeta^f(\tau), \zeta^c(\tau)\right)_h - \hat{\psi}\left(\hat{y}_0', \hat{y}_H, \zeta^f(\tau + 1), \zeta^c(\tau)\right)_h}
    \leq C_0 \lambda_0^{\abs{h - \tau}} \norm{\zeta_\tau^f - (\zeta_\tau^f)'}
\end{align}
holds for all $\tau = \{1, \ldots, H-1\}$, and the two corner cases
\begin{align}
    \norm{\hat{\psi}\left(\hat{y}_0, \hat{y}_H, \zeta^f(1), \zeta^c(0)\right)_h - \hat{\psi}\left(\hat{y}_0', \hat{y}_H, \zeta^f(1), \zeta^c(0)\right)_h} \leq{}& C_0 \lambda_0^{h} \norm{\hat{y}_0- \hat{y}_0'},\label{thm:SOCO-sensitivity-e4}\\
    \norm{\hat{\psi}\left(\hat{y}_0', \hat{y}_H, \zeta^f(H), \zeta^c(H)\right)_h - \hat{\psi}\left(\hat{y}_0', \hat{y}_H', \zeta^f(H), \zeta^c(H)\right)_h} \leq{}& C_0 \lambda_0^{H - h} \norm{\hat{y}_H- \hat{y}_H'}.\label{thm:SOCO-sensitivity-e5}
\end{align}
Using the triangle inequality to combine \eqref{thm:SOCO-sensitivity-e2}, \eqref{thm:SOCO-sensitivity-e3}, \eqref{thm:SOCO-sensitivity-e4}, \eqref{thm:SOCO-sensitivity-e5}, we see that
\begin{align*}
    &\norm{\hat{\psi}\left(\hat{y}_0, \hat{y}_\horizonvar, \zeta_{1:H-1}^f, \zeta_{0:H-1}^c\right)_h - \hat{\psi}\left(\hat{y}_0', \hat{y}_\horizonvar', (\zeta_{1:H-1}^f)', (\zeta_{0:H-1}^c)'\right)_h}\\
    \leq{}& \norm{\hat{\psi}\left(\hat{y}_0, \hat{y}_H, \zeta^f(1), \zeta^c(0)\right)_h - \hat{\psi}\left(\hat{y}_0', \hat{y}_H, \zeta^f(1), \zeta^c(0)\right)_h}\\
    &+ \sum_{\tau = 1}^{H-1} \norm{\hat{\psi}\left(\hat{y}_0', \hat{y}_H, \zeta^f(\tau), \zeta^c(\tau)\right)_h - \hat{\psi}\left(\hat{y}_0', \hat{y}_H, \zeta^f(\tau + 1), \zeta^c(\tau)\right)_h}\\
    &+ \sum_{\tau = 0}^{H-1} \norm{\hat{\psi}\left(\hat{y}_0', \hat{y}_H, \zeta^f(\tau + 1), \zeta^c(\tau)\right)_h - \hat{\psi}\left(\hat{y}_0', \hat{y}_H, \zeta^f(\tau + 1), \zeta^c(\tau + 1)\right)_h}\\
    &+ \norm{\hat{\psi}\left(\hat{y}_0', \hat{y}_H, \zeta^f(H), \zeta^c(H)\right)_h - \hat{\psi}\left(\hat{y}_0', \hat{y}_H', \zeta^f(H), \zeta^c(H)\right)_h}\\
    \leq{}& C_0\bigg(\decayvar_0^{h}\norm{\hat{y}_0 - \hat{y}_0'} + \sum_{\tau=1}^{\horizonvar-1} \decayvar_0^{\abs{h - \tau}}\norm{\zeta_\tau^f - (\zeta_\tau^f)'} + \sum_{\tau = 0}^{\horizonvar-1}\decayvar_0^{\abs{h - \tau}}\norm{\zeta_\tau^c - (\zeta_\tau^c)'} + \decayvar_0^{\horizonvar-h}\norm{\hat{y}_\horizonvar - \hat{y}_\horizonvar'} \bigg).
\end{align*}

==> Proofs/obsolete/general-constrained.tex <==
Consider the following special case of problem \eqref{equ:online_control_problem}:
\begin{align}\label{equ:constrained-LQR-known}
    \min_{x_{0:T}, u_{0:T-1}} &\sum_{t = 0}^{T-1} \left( (x_t - \bar{x}_t)^\top Q_t (x_t - \bar{x}_t) + u_t^{\top} R_t u_t \right) + (x_T - \bar{x}_T(\xi_T))^\top Q_T(\xi_T) (x_T - \bar{x}_T(\xi_T)) \nonumber\\*
    \text{ s.t. }& x_t = A_t\cdot x_t + B_t\cdot u_t + w_t,~ \forall 0 \leq t < T,\nonumber\\*
    & \tilde{\varGamma}^x_t x_t + \tilde{\varGamma}^u_t u_t \geq \tilde{\gamma}_t,~ \forall 0 \leq t < T,\nonumber\\*
    &x_0 = x(0),
\end{align}
where $\tilde{\varGamma}^x_t \in \mathbb{R}^{r_t \times n}$ and $\tilde{\varGamma}^u_t \in \mathbb{R}^{r_t \times m}$ are constraint matrices on $x$ and $u$, respectively, and $\tilde{\gamma} \in \mathbb{R}^{r_t}$ ($r_t$ is the number of constraints). Our result relies on a critical lemma (Proposition 4 in \cite{xu2019exponentially}), for which we need to introduce some preliminaries first. We remind the reader that we change the notations to make the paper coherent. \yang{I'm not sure whether we should stick to the notations in the original paper. They overload some of the letters we use, and use too many capital letters. But changing them might make the readers confused how to prove the lemma.}

For a specific instance derived from \eqref{equ:constrained-LQR-known}, it is critical to identify which constraints are active in the optimal solution (note that in \eqref{equ:constrained-LQR-known}, constraint matrices are marked by tilde, indicating that they might not be active). More specifically, suppose $I_t \subseteq \lbrace 1,\ldots,r_t \rbrace$ is the index set for active constraints at time step $t$, and define the corresponding active constraint matrices as $\varGamma^x_{t,I_t} := \tilde{\varGamma}^x_t(I_t, :)$, $\varGamma^u_{t,I_t} := \tilde{\varGamma}^u_t(I_t, :)$, $\gamma_t := \tilde{\gamma}_t(I_t)$. We additionally define $\hat{\varGamma}^u_{t,I_t} := (\varGamma^u_{t,I_t} R_t^{-1} (\varGamma^u_{t,I_t})^{\top})^{-1}$ (for the case $I_t = \varnothing$, let $\hat{\varGamma}^u_{t,I_t} = 0$). 

\begin{assumption}\label{assump:general-constrained}
  We make the following assumptions on the system:
  \begin{enumerate}
      \item (well-conditioned costs) The cost matrices are uniformly bounded by $\norm{Q_t} \leq \overline{q}I$, $\norm{R_t} \leq \overline{r}I$, $Q_t \succeq \underline{q}I$, $R_t \succeq \underline{r}I$ with constants $\underline{q},\overline{q},\underline{r},\overline{r}$ independent of the time step $t$.
      
      \item (Lipschitz dynamics) The dynamical matrices are uniformly bounded by $\norm{A_t} \leq a$, $\norm{B_t} \leq b$ with constants $a,b$ independent of the time step $t$.
      
      \item ($(d, \sigma)$-uniform controllability) There exists a positive constant $\sigma$ such that $\sigma_{\min} \left( M(t, d) \right) \geq \sigma$ holds for all time steps $t = 0, \ldots, T - d$, where $d$ denotes the controllability index.
      
      \item (bounded constraint matrices) The active constraint matrices are uniformly upper bounded by $\norm{\varGamma^x_{t,I_t}} \leq c_x$, $\norm{\varGamma^u_{t,I_t}} \leq c_u$, $\norm{\hat{\varGamma}^u_{t,I_t}} \leq \hat{c}_u$ for constants $c_x,c_u,\hat{c}_u$ independent of the active index set $I_t$ and time step $t$.
      
      \item ($\gamma$-uLICQ constraints) There exists a positive constant $\gamma$ such that $\varGamma^u_{t,I^*_t} (\varGamma^u_{t,I^*_t})^{\top} \succeq \gamma I$ for all time steps $t = 0, \ldots, T$, where $I^*_t \subseteq \lbrace 1,\ldots,r_t \rbrace$ is the active index set along the offline optimal trajectory $\{x^*_t\}$. Further, there exists a uniform radius $R$ such that, for any $x_t \in \mathcal{B}(x^*t, R)$, the active index set is $I^*_t$.
  \end{enumerate}
\end{assumption}

We point out that, in \cite{xu2019exponentially}, assumption (3) is referred to as UCC($\lambda_C$) ($\lambda_C$-uniformly completely controllable) in \cite{xu2019exponentially}, where $\lambda_C = \sigma^2$, and assumption (5) is referred to as UDB($\lambda_H$) ($\lambda_H$-uniformly bounded from below) , where $\lambda_H = \gamma$. The terminology we use is more common in control and optimization literature \cite{shin2020decentralized, shin2021controllability}.

Now we are ready to apply Proposition 4 in \cite{xu2019exponentially} to get the following lemma.

\begin{lemma}\label{lemma:perturbation:general-constrained}
  Under Assumption \ref{assump:general-constrained}, the FTOCP $\psi_{t_1}^{t_2}(z, \xi^*_{t_1:t_2}; F_{t_2})$ satisfies
  \begin{equation}\label{equ:perturbation:general-constrained:e1}
    \begin{aligned}
      \norm{\psi_{t_1}^{t_2}(z, \xi_{t_1:t_2}^*; F_{t_2})_{y_h} - \psi_{t_1}^{t_2}(z', \xi_{t_1:t_2}^*; F_{t_2})_{y_h}} &\leq C \decayvar^{h-t_1} \norm{z - z'},\\
      \norm{\psi_{t_1}^{t_2}(z, \xi_{t_1:t_2}^*; F_{t_2})_{v_h} - \psi_{t_1}^{t_2}(z', \xi_{t_1:t_2}^*; F_{t_2})_{v_h}} &\leq C \decayvar^{h-t_1} \norm{z - z'},
    \end{aligned}
  \end{equation}
  and
  \begin{equation}\label{equ:perturbation:general-constrained:e2}
    \begin{aligned}
      \norm{\psi_{t_1}^{t_2}(z, \xi_{t_1:t_2}; F_{t_2})_{y_h} - \psi_{t_1}^{t_2}(z', \xi'_{t_1:t_2}; F_{t_2})_{y_h}} &\leq \cdots \norm{\xi-\xi'},\\
      \norm{\psi_{t_1}^{t_2}(z, \xi_{t_1:t_2}^*; F_{t_2})_{v_h} - \psi_{t_1}^{t_2}(z', \xi'_{t_1:t_2}; F_{t_2})_{v_h}} &\leq \cdots \norm{\xi-\xi'},
    \end{aligned}
  \end{equation}
  where the constants are determined by (recall that $d$ is the controllability index of the system)
  \begin{gather*}
      \alpha = a + \frac{b c_x c_u \hat{c}_u}{\underline{r}},~
      \beta = b + \frac{b c_u^2 \hat{c}_u}{\underline{r}},\\
      \mu = \frac{\beta (1-\alpha^d)}{1-\alpha},~
      \eta = q \left( 1 + \sum_{i=1}^{d-1} \left( \alpha^i + \frac{\mu^2}{\sigma^2} \alpha^d \right)^2 \right) + \frac{r\mu^2}{\sigma^2} \alpha^{2d},\\
      C = \max\left\lbrace 1, \frac{c_x c_u \hat{c}_u}{\underline{q}} + \frac{\alpha b \gamma (\underline{r} + \beta^2 \gamma)(\underline{r} + c_u^2 \hat{c}_u)}{\underline{r}^3} \right\rbrace \sqrt{\frac{\gamma}{\underline{q}}},~
      \decayvar = \frac{1}{\sqrt{1+\underline{q} / \gamma}}.
  \end{gather*}
\end{lemma}

\begin{proof}[Proof of \Cref{lemma:perturbation:general-constrained}]
  For \eqref{equ:perturbation:general-constrained:e1}, recall that using Proposition 4 in \cite{xu2019exponentially} we have
  \begin{equation}\label{equ:perturbation:general-constrained-proof:e1}
      \norm{\nabla_{z} \psi_{t_1}^{t_2}(z, \xi^*_{t_1:t_2}; F_{t_2})_{y_h}} \leq C \decayvar^{h-t},~
      \norm{\nabla_{z} \psi_{t_1}^{t_2}(z, \xi^*_{t_1:t_2}; F_{t_2})_{v_h}} \leq C \decayvar^{h-t},
  \end{equation} we only have to notice that
  \begin{align*}
      \norm{\psi_{t_1}^{t_2}(z, \xi_{t_1:t_2}^*; F_{t_2})_{y_h} - \psi_{t_1}^{t_2}(z', \xi_{t_1:t_2}^*; F_{t_2})_{y_h}}
      &= \norm{\int_{0}^{1} \left( \frac{\diff}{\diff \theta} \psi_{t_1}^{t_2}(z + \theta(z'-z), \xi_{t_1:t_2}^*; F_{t_2})_{y_h}\right) \diff \theta} \\
      &= \norm{\int_{0}^{1} \left( \nabla_{z} \psi_{t_1}^{t_2}(z+\theta(z'-z), \xi^*_{t_1:t_2}; F_{t_2})_{y_h} \right)^{\top} (z'-z) \diff \theta} \\
      &\leq \int_{0}^{1} \norm{\nabla_{z} \psi_{t_1}^{t_2}(z+\theta(z'-z), \xi^*_{t_1:t_2}; F_{t_2})_{y_h}} \norm{z-z'} \diff \theta \\
      &\leq C \lambda^{h-t_1} \norm{z-z'}.
  \end{align*}
  the proof for $\psi_{t_1}^{t_2}(z, \xi_{t_1:t_2}^*; F_{t_2})_{v_h}$ is similar. This finishes the proof of the first part.
  
  For \eqref{equ:perturbation:general-constrained:e2}, we need a slight variation of the results in Proposition 4 in \cite{xu2019exponentially}.
\end{proof}

==> Proofs/obsolete/general-nonlinear.tex <==
\yang{We desperately need to clean up our notations. Too messy and not consistent among chapters (e.g., 3.2 and 4.2 use completely different notations on KKT matrices.}

Consider the general unconstrained form of problem \eqref{equ:online_control_problem}:
\begin{align}\label{equ:unconstrained-nonlinear-known}
    \min_{x_{0:t_2}, u_{0:t_2-1}} &\sum_{t=t_1}^{t_2-1} f_t(x_t, u_t; \xi_t^*) + F_{t_2}(x_{t_2}; \xi_{t_2}^*) \nonumber\\*
    \text{ s.t. }&x_{t+1} = g_t(x_t, u_t; \xi_t^*), &\forall t_1 \leq t < t_2,\nonumber\\*
    &x_0 = x(0),
\end{align}
where $f_t$, $g_t$ and $F_{t_2}$ are assumed to be twice-continuously differentiable. We need to introduce some preliminaries first.


The corresponding FTOCP $\psi_{t_1}^{t_2}$ can be viewed as a convex optimization problem over $x_{t_1:t_2}$ and $u_{t_1:t_2-1}$ with dynamics equations as equality constraints (note that we eliminate the initial state constraint), for which it is intuitive to apply the KKT condition. More specifically, let $\xu_0 = u_0$, $\xu_t = [x_t, u_t]$ (for $t = t_1,\cdots,t_2-1$), $\xu_{t_2} = x_{t_2}$, and $\xu = [\xu_{t_1}, \xu_{t_1+1}, \cdots, \xu_{t_2}]$ be an ordered collection of all decision variables. Let $f(\xu; \xi) = \sum_{t=t_1}^{t_2-1} f_t(\xu_t; \xi_t^*) + F_{t_2}(\xu_{t_2}; \xi_t^*)$ denote the objective function (note that $x_0 = z$ is given), and define $\tilde{g}_{t+1}(\xu_{t:t+1}; \xi_t^*) = x_{t+1} - g_t(x_t, u_t; \xi_t^*)$ (for $t = t,\cdots,T-1$) so that the constraints can be written uniformly as $\tilde{g} := [\tilde{g}_{t_1+1}, \cdots, \tilde{g}_{t_2}] = 0$. Let $\lagr = [\lagr_{t_1+1}, \cdots, \lagr_{t_2}]$ be the vector of Lagrangian multipliers corresponding to $\tilde{g}_{t_1+1}, \cdots, \tilde{g}_{t_2}$. In this way, we can write the Lagrangian as $\mathcal{L}(\xu, \lagr; \xi) = f(\xu; \xi) + \lagr^{\top} \tilde{g}(\xu; \xi)$. The Hessian of the Lagrangian can be written as $H(\xu, \lagr;\xi) := \nabla^2_{\xu\xu} \mathcal{L}(\xu, \lagr; \xi) = \diag(H_0, H_1, \cdots, H_t)$, where
\begin{gather*}
    H_{t_1}(\xu_{t_1}; \xi_{t_1}) = \nabla^2_{u_{t_1} u_{t_1}} \mathcal{L}(\xu_{t_1}; \xi_{t_1}) = \nabla^2_{u_{t_1} u_{t_1}} f_{t_1}(\xu_{t_1}; \xi_{t_1}), \\
    H_t(\xu_t, \lagr_t; \xi_t) =
    \begin{bmatrix}
      \nabla^2_{x_t x_t} \mathcal{L}(\xu, \lagr; \xi) & \nabla^2_{x_t u_t} \mathcal{L}(\xu, \lagr; \xi) \\
      \nabla^2_{u_t x_t} \mathcal{L}(\xu, \lagr; \xi) & \nabla^2_{u_t u_t} \mathcal{L}(\xu, \lagr; \xi)
    \end{bmatrix}, t=t_1+1,\cdots,t_2-1, \\
    H_{t_2}(\xu_{t_2}; \xi_{t_2}) = \nabla^2_{x_{t_2} x_{t_2}} \mathcal{L}(\xu_{t_2}; \xi_{t_2}) = \nabla^2_{x_{t_2} x_{t_2}} F_{t_2}(\xu_{t_2}; \xi_{t_2}).
\end{gather*}
Further, define $A_t := \nabla_{x_t}^{\top} g_t(\xu_t; \xi_t)$, $B_t := \nabla_{u_t}^{\top} g_t(\xu_t; \xi_t)$, and the Jacobian of the constraints can be written as
\begin{equation*}
    G(\xu; \xi) := \nabla_{\xu} \tilde{g}(\xu; \xi) =
    \left[ \begin{smallmatrix}
      -B_{t_1} & I \\
      & -A_{t_1+1} & -B_{t_1+1} & I \\
      & & \ddots & \ddots & \ddots \\
      & & & & -A_{t_2-1} & -B_{t_2-1} & I
    \end{smallmatrix} \right].
\end{equation*}
To introduce the uSOSC assumption, we also introduce the reduced Hessian: let $Z$ be the null-space matrix of $G$ (i.e., the column vectors of $Z$ form an orthonormal basis of the null space of $G$), and the \textit{reduced Hessian} $\Hre(\xu, \lagr; \xi) := Z^{\top} H Z$. We also define the KKT matrix of the Lagrangian as
\begin{equation*}
    K = \begin{bmatrix}
      H & G^{\top} \\
      G 
    \end{bmatrix}.
\end{equation*}

\begin{assumption}\label{assump:general-nonlinear}
  We make the following assumptions on the system:
  \begin{enumerate}
      \item (well-conditioned costs) The cost functions in $\{f_t\}_{0\leq t\leq T-1} \cup \{F_{t_2}\}$ are non-negative, $\mu_f$-strongly convex, $\ell_f$-smooth, and in $C^2$. Further, we assume their minimizers are at $0$ without loss of generality.
      
      \item (well-conditioned dynamics) The dynamical functions in $\{g_t\}_{0\leq t\leq T-1}$ are $\mu_g$-strongly convex, $\ell_g$-smooth, and in $C^2$.
      
      \item (Lipschitz dynamics) There exists a radius $R > 0$, such that for any time step $t$ and $(\xu_t, \lagr_t) \in \mathcal{B}((\xu^*_t, \lagr^*_t), R)$, the linearized dynamical matrices at $\xu_t$ are uniformly bounded by $\norm{A_t(\xu_t; \xi_t)} \leq a$, $\norm{B_t(\xu_t; \xi_t)} \leq b$ with constants $a,b$ independent of time step $t$, $\xi_t$ and the choice of $\xu_t$.
      
      \item ($(d, \sigma)$-uniform controllability) There exists a positive constant $\sigma$ such that $\sigma_{\min} \left( M(t, d) \right) \geq \sigma$ holds for all time steps $t = 0, \ldots, T - d$, where $d$ denotes the controllability index.
      
      \item (trajectory mismatch) The trajectory formed by minimizers of stage costs (i.e., $0,0,\cdots$) satisfy
      \[\norm{\tilde{g}(0,0; \xi^*)} \leq D_{traj}.\]
  \end{enumerate}
\end{assumption}

We point out that, for assumption (3), readers could refer to \Cref{def:controllability} for the definition of controllability matrix $M(t,d)$, where the $A_t$ and $B_t$ matrices for non-linear systems are understood as local linearizations of $g_t$, and $M$ is evaluated at a fixed point $z$ with parameter $\xi$.

We now show some technical results that $H$, $G$ and $\lagr^*$ are all bounded.

\begin{lemma}\label{lemma:general-nonlinear:bounded-H-G-lagr}
    The following results hold:
    \begin{enumerate}[nosep, leftmargin=1em]
        \item There exists constants $0 < \underline{\sigma}_G < \overline{\sigma}_G$ such that $\underline{\sigma}_G I \preceq G \preceq \overline{\sigma}_G I$.
        
        \item The optimal primal-dual solution $(\xu^*, \lagr^*)$ is bounded by $\norm{\xu^*} \leq \frac{2L}{\mu_f \underline{\sigma}_G} D_{traj}$, $\norm{\lagr^*} \leq \frac{2}{\mu_f} (\frac{L}{\underline{\sigma}_G})^2 D_{traj}$, where $f$ is $L$-smooth and $\mu_f$-strongly convex.
        
        \item If $D_{traj} \leq \frac{\mu_f^2}{2 \mu_g (\frac{L}{\underline{\sigma}_G})^2}$, then there exists constants $0 < \underline{\sigma}_H < \overline{\sigma}_H$ such that $\underline{\sigma}_H I \preceq H \preceq \overline{\sigma}_H I$.
    \end{enumerate}
\end{lemma}

\begin{proof}
    (1) The upper bound follows from Lipschitzness of dynamics, while the lower bound follows from $(d,\sigma)$-uniform controllability and Lipschitz dynamics (see Lemma 12 in \cite{shin2021controllability}).
    
    (2) By optimality we have $\mathcal{L}(\xu^*, \lagr^*; \xi)$, which expands to
    \begin{align*}
        f(\xu^*; \xi) &= f(\xu^*; \xi) + (\lagr^*)^{\top} \tilde{g}(\xu^*; \xi) \\
        &\leq f(0; \xi) + (\lagr^*)^{\top} \tilde{g}(0; \xi) \\
        &\leq f(\xu^*; \xi) - \frac{\mu}{2} \norm{\xu^*}^2 + (\lagr^*)^{\top} \tilde{g}(0; \xi),
    \end{align*}
    so we have $\frac{\mu}{2} \norm{\xu^*}^2 \leq (\lagr^*)^{\top} \tilde{g}(0; \xi)$. Meanwhile, by KKT condition we have $\nabla_{\xu} f(\xu^*; \xi) + \left( \nabla_{\xu} g(\xu^*; \xi) \right)^{\top} \lagr^* = 0$, and by optimality we have $\nabla_{\xu} f(0; \xi) = 0$, which expands to
    \begin{align*}
        \underline{\sigma}_G \norm{\lagr^*}
        \leq \norm{\left( \nabla_{\xu} \tilde{g}(\xu^*; \xi) \right)^{\top} \lagr^*}
        = \norm{\nabla_{\xu} f(\xu^*; \xi)}
        \leq L \norm{\xu^*}
        \leq L \sqrt{\frac{2}{\mu} \norm{\lagr^*} \norm{\tilde{g}(0; \xi)}},
    \end{align*}
    or equivalently, $\norm{\lagr^*} \leq \frac{2}{\mu} (\frac{L}{\underline{\sigma}_G})^2 D_{traj}$. Hence $\norm{\xu^*} \leq \frac{2}{\mu} \norm{\lagr^*} \norm{\tilde{g}(0;\xi)} \leq \frac{2L}{\mu_f \underline{\sigma}_G} D_{traj}$.
    
    (3) This directly follows from (2), when we take $\underline{\sigma}_H = \mu_f - \norm{\eta^*} \mu_g$ and $\overline{\sigma}_H = L_f + \norm{\eta^*} L_g$.
\end{proof}

We will introduce a lemma that characterizes the structure of $K^{-1}$ (which is similar to Lemma 2 in \cite{na2020superconvergence}). To make the exponential decaying result more intuitive, we will adopt the same rearranging protocol as used in Section 4.2 (i.e., rearrange $(\xu, \lagr)$ to be $(\xu_{t_1}, \xu_{t_1+1}, \lagr_{t_1+1}, \cdots, \xu_{t_2}, \lagr_{t_2})$. Recall that we have removed $x_0$ (which is fixed by prescribed parameter $z$ of the problem), so that the matrix would look like
\begin{equation*}
    \left[\begin{array}{c|ccc|ccc|cc}
        R_{t_1} & & & - B_{t_1}^{\top} & & & & & \\
        \hline
        & Q_{t_1+1} & & I & & & -A_{t_1+1}^{\top} & & \\
        & & R_{t_1+1} & & & & - B_{t_1+1}^{\top} & & \\
        - B_{t_1} & I & & & & & & & \\
        \hline
        & & & & Q_{t_1+2} & & I & & -A_{t_1+2}^{\top} \\
        & & & & & R_{t_1+2} & & & -B_{t_1+2}^{\top} \\
        & -A_{t_1+1} & -B_{t_1+1} & & I & & & & \\
        \hline
        & & & & & & & P & I\\
        & & & & -A_{t_1+2} & -B_{t_1+2} & & I &
    \end{array}\right],
\end{equation*}
which is block-tridiagonal and thus shows a exponential decay property. For simplicity, we will rearrange the vector back to $(\xu, \lagr)$, and will work under the convention that $K^{-1}$ is partitioned as follows:
\begin{equation}\label{equ:general-nonlinear:K-inverse-block}
    K^{-1} =:
    \left[ \begin{array}{ccc:ccc}
      K^{-1}_{(t_1,t_1),1} & \cdots & K^{-1}_{(t_1,t_2),1} & K^{-1}_{(t_1,t_1),2} & \cdots & K^{-1}_{(t_1,t_2-1),2} \\
      \vdots & \ddots & \vdots & \vdots & \ddots & \vdots \\
      K^{-1}_{(t_2,t_1),1} & \cdots & K^{-1}_{(t_2,t_2),1} & K^{-1}_{(t_2,t_1),2} & \cdots & K^{-1}_{(t_2,t_2-1),2} \\\hdashline
      (K^{-1}_{(t_1,t_1),2})^{\top} & \cdots & (K^{-1}_{(t_2,t_1),2})^{\top} & K^{-1}_{(t_1,t_1),3} & \cdots & K^{-1}_{(0,t_2-1),3} \\
      \vdots & \ddots & \vdots & \vdots & \ddots & \vdots \\
      (K^{-1}_{(t_2,t_2-1),2})^{\top} & \cdots & (K^{-1}_{(t_2,t_2-1),2})^{\top} & K^{-1}_{(t_2,t_1),3} & \cdots & K^{-1}_{(t_2,t_2-1),3}
    \end{array} \right]
\end{equation}
Now we have the following lemma characterizing the structure of $K^{-1}$.

\begin{lemma}
  Under Assumption \ref{assump:general-nonlinear}, the KKT matrix $K$ of the FTOCP $\psi_{t_1}^{t_2}(\xu, \xi_{t_1:t_2}; F_{t_2})$ satisfies
  \begin{equation}\label{equ:perturbation:general-nonlinear:e1}
      \norm{K^{-1}_{(i,j),1}} \leq C_0 \lambda_0^{|i-j|},~
      \norm{K^{-1}_{(i,j),2}} \leq C_0 \lambda_0^{|i-j|},~
      \norm{K^{-1}_{(i,j),3}} \leq C_0 \lambda_0^{|i-j|}
  \end{equation}
  for $i=0,\cdots,T$ and $j=0,\cdots,T-1$. 
\end{lemma}

\begin{proof}
  By \Cref{lemma:general-nonlinear:bounded-H-G-lagr}, the singular spectrum of $H$ and $G$ are bounded from both sides, and this is a direct corollary of \Cref{lemma:block-singular-value}.
\end{proof}

\yang{Caution: misuse of notations. We might have to use a different notation, either for the initial state $z$, or for the primal-dual solution $\xu^*$.}

\begin{lemma}\label{lemma:perturbation:general-nonlinear}
  Under Assumption \ref{assump:general-nonlinear}, the optimal solution of the FTOCP satisfies
  \begin{equation}\label{equ:perturbation:general-nonlinear:e2}
    \begin{aligned}
      \norm{\psi_{t_1}^{t_2}(z, \xi_{t_1:t_2}; F_{t_2})_{y_h} - \psi_{t_1}^{t_2}(z', \xi'_{t_1:t_2}; F_{t_2})_{y_h}} &\leq C \left( \decayvar^{h-t} \norm{z - z'} + \sum_{t=t_1}^{t_2} \lambda^{|h-t|} \norm{\xi_t - \xi'_t} \right),\\
      \norm{\psi_{t_1}^{t_2}(z, \xi'_{t_1:t_2}; F_{t_2})_{v_h} - \psi_{t_1}^{t_2}(z', \xi_{t_1:t_2}; F_{t_2})_{v_h}} &\leq C \left( \decayvar^{h-t} \norm{z - z'} + \sum_{t=t_1}^{t_2} \lambda^{|h-t|} \norm{\xi_t - \xi'_t} \right),
    \end{aligned}
  \end{equation}
  where the constants are given by
  \begin{gather*}
      C = \left( \ell_f + \frac{2}{\mu_f} (\frac{L}{\underline{\sigma}_G})^2 D_{traj} \ell_g \right) C_0,~
      \ell = \ell_0.
  \end{gather*}
\end{lemma}

\begin{proof}[Proof of \Cref{lemma:perturbation:general-nonlinear}]
We use an approach similar to the proof of Theorem 3.1 in \cite{lin2021perturbation}. More specifically, consider a small perturbation to the system parameters $\zeta := (z, \xi_{t_1:t_2})$ in the form $\zeta' = \zeta + \theta e$, where $\theta \in \mathbb{R}$ represents the magnitude of the perturbation, and vector $e = [e_0^{\top}, \delta^{\top}]^{\top}$ characterizes the direction of perturbation (where $e_0 \in \mathbb{R}^n$ perturbs initial state $z' = z + \theta e_0$, while $\delta = [\delta_t, \ldots, \delta_{t_2}]$ perturbs $\xi'_{t_1:t_2} = \xi_{t_1:t_2} + \theta \delta$). Let $(\xu^*(\zeta), \lagr^*(\zeta))$ denote the optimal primal-dual solution of \eqref{equ:unconstrained-nonlinear-known} given parameter $\zeta$. The KKT condition guarantees that, for any $\theta \in \mathbb{R}$,
\begin{equation*}
    \nabla_{\xu} \mathcal{L}(\xu^*(\zeta'), \lagr^*(\zeta'), \zeta') = 0,~
    \tilde{g}(\xu^*(\zeta'), \zeta') = 0.
\end{equation*}
Now take derivative with respect to $\theta$, and we have
\begin{align}
    0 &= \frac{\diff}{\diff \theta} \Big( \nabla_{\xu} f(\xu^*(\zeta'), \zeta') + (\nabla_{\xu} \tilde{g}(\xu^*(\zeta'), \zeta'))^{\top} \lagr^*(\zeta') \Big) \nonumber\\
    &= \nabla^2_{\xu\xu} f(\xu^*(\zeta'), \zeta') \frac{\diff \xu^*(\zeta')}{\diff \theta}
       + \nabla^2_{\xu \zeta} f(\xu^*(\zeta'), \zeta') \frac{\diff \zeta'}{\diff \theta}
       + \nabla_{\xu} \tilde{g}(\xu^*(\zeta'), \zeta'))^{\top} \frac{\diff \lagr^*(\zeta')}{\diff \theta} \nonumber\\
    &\qquad {}+ \sum_{t=t_1+1}^{t_2}\lagr^*_i(\zeta') \left( \nabla^2_{\xu\xu} \tilde{g}_i(\xu^*(\zeta‘), \zeta') \frac{\diff \xu^*(\zeta')}{\diff \theta} + \nabla^2_{\xu \zeta} \tilde{g}_i(\xu^*(\zeta’), \zeta') \frac{\diff \zeta'}{\diff \theta} \right) \nonumber\\
    &= H(\xu^*(\zeta'), \lagr^*(\zeta'), \zeta') \frac{\diff \xu^*(\zeta')}{\diff \theta}
       + G(\xu^*(\zeta'), \zeta')^{\top} \frac{\diff \lagr^*(\zeta')}{\diff \theta}
       + \nabla^2_{\xu \zeta} \mathcal{L}(\xu^*(\zeta'), \lagr^*(\zeta'), \zeta') \frac{\diff \zeta'}{\diff \theta}, \label{lemma:perturbation:general-nonlinear:lagrange-1}\\
    0 &= \frac{\diff}{\diff \theta} \tilde{g}(\xu^*(\zeta'), \zeta') 
    = G(\xu^*(\zeta'), \zeta') \frac{\diff \xu^*(\zeta')}{\diff \theta} + \nabla_{\zeta} \tilde{g}(\xu^*(\zeta'), \zeta')^{\top} \frac{\diff \zeta'}{\diff \theta}. \label{lemma:perturbation:general-nonlinear:lagrange-2}
\end{align}
To simplify the notation, we define the following $(t_2-t_1+1) \times 1$ block matrices
\begin{gather*}
    R^{(z)} := - \nabla_{z} \nabla_{\xu_{t_1:t_2}} \mathcal{L}(\xu^*(\zeta'), \zeta'),\quad
    R^{(\zeta_t)} := - \nabla_{\zeta_t} \nabla_{\xu_{t_1:t_2}} \mathcal{L}(\xu^*(\zeta'), \zeta'), \forall t_1 \leq t \leq t_2\\
    S^{(z)} := - \nabla_{z} \tilde{g}(\xu^*(\zeta'), \zeta'),\quad
    S^{(\zeta_t)} := - \nabla_{\zeta_t} \tilde{g}(\xu^*(\zeta'), \zeta'), \forall t_1 \leq t \leq t_2,
\end{gather*}
where block sizes in $R^{(z)}$ and $S^{(z)}$ are $n\times n$, while block sizes in $R^{(\zeta_t)}$ and $S^{(\zeta_t)}$ are $n\times d$. By the coupling properties of the Lagrangian, we know that only the 1st block of $R^{(z)}$, $S^{(z)}$, and the $t$th and ($t+1$)th blocks of $R^{(\zeta_t)}, S^{(\zeta_t)}$, could be non-zero.

Now we have, equivalent to equations \eqref{lemma:perturbation:general-nonlinear:lagrange-1} and \eqref{lemma:perturbation:general-nonlinear:lagrange-2},
\begin{gather*}
    H(\xu^*(\zeta'), \lagr^*(\zeta'), \zeta') \frac{\diff \xu^*(\zeta')}{\diff \theta} + G(\xu^*(\zeta'), \zeta')^{\top} \frac{\diff \lagr^*(\zeta')}{\diff \theta}
    = - R^{(z)} e_0 - \sum_{t=t_1}^{t_2} R^{(\zeta_t)} \delta_t, \\
    G(\xu^*(\zeta'), \zeta') \frac{\diff \xu^*(\zeta')}{\diff \theta} = - - S^{(z)} e_0 - \sum_{t=t_1}^{t_2} S^{(\zeta_t)} \delta_t,
\end{gather*}
or in more compact form,
\begin{equation}\label{lemma:perturbation:general-nonlinear:matrix-form}
    \begin{bmatrix}
        \tfrac{\diff}{\diff \theta} \xu^*(\zeta + \theta e) \\
        \tfrac{\diff}{\diff \theta} \lagr^*(\zeta + \theta e)
    \end{bmatrix}
    = -K^{-1} \left( \begin{bmatrix}
        R^{(z)} \\
        S^{(z)}
    \end{bmatrix} e_0 + \sum_{t=t_1}^{t_2} \begin{bmatrix}
        R^{(\zeta_t)} \\
        S^{(\zeta_t)}
    \end{bmatrix} \delta_t \right).
\end{equation}
Therefore, the $h$th entry of $\frac{\diff}{\diff \theta} \xu^*(\zeta + \theta e)$ is
\begin{align}
    \frac{\diff}{\diff \theta} \xu^*(\zeta + \theta e)_{h}
    ={}& - \left( K^{-1}_{(h,t),1} R^{(z)}_{(1,1)} + K^{-1}_{(h,t),2} S^{(z)}_{(1,1)} \right) e_0 \nonumber\\
      &{}- \sum_{t=t_1}^{t_2} \left( K^{-1}_{(h,t:t+1),1} R^{(\zeta_t)}_{(t:t+1,1)} + K^{-1}_{(h,t:t+1),2} S^{(\zeta_t)}_{(t:t+1,1)} \right) \delta_t.
\end{align}
Since $f_t$ and $g_t$ are all $\ell_f$- and $\ell_g$- smooth in all variables, and by \Cref{lemma:general-nonlinear:bounded-H-G-lagr}, matrices $R^{(z)}_{(1,1)}$, $S^{(z)}_{(1,1)}$, $R^{(\zeta_t)}_{(t:t+1,1)}$ and $S^{(\zeta_t)}_{(t:t+1,1)}$ are all bounded by $\ell_f + \frac{2}{\mu_f} (\frac{L}{\underline{\sigma}_G})^2 D_{traj} \ell_g$. Hence we have
\begin{equation}
    \norm{\frac{\diff}{\diff \theta} \psi(\zeta + \theta e)_{h}}
    \leq \norm{\frac{\diff}{\diff \theta} \xu^*(\zeta + \theta e)_{h}}
    \leq C \left( \decayvar^{h} \norm{e_0} + \sum_{t=t_1}^{t_2} \decayvar^{|h-t|} \norm{\delta_t} \right).
\end{equation}
Then by integration, we have
\begin{align*}
    \norm{\psi(\zeta)_h - \psi(\zeta + e)_h}
    ={}& \norm{\int_{0}^{1} \frac{\diff}{\diff \theta} \psi(\zeta + \theta e)_{h} \diff \theta}\\
    \leq{}& \int_0^1 \norm{\frac{\diff}{\diff \theta} \psi(\zeta + \theta e)_{h}} \diff \theta\\
    \leq{}& C \left( \decayvar^{h} \norm{e_0} + \sum_{t=t_1}^{t_2} \decayvar^{|h-t|} \norm{\delta_t} \right).
\end{align*}
This finishes the proof.
\end{proof}

\yang{Subscripts are very messy here. It is better that we force the FTOCP problem to start from 0 or 1. If we still want to use subscript $y_t$ or $v_t$ directly, it would be very bad notation in matrices.}

==> Proofs/switching-cost-opt-sol.tex <==
By Assumption \ref{assump:controllability}, since $t_2 - t_1 \geq d$, we know the optimization problem $\psi_{t_1}^{t_2}$ is feasible for all parameter tuple
\[\upsilon_{t_1}^{t_2} \in \mathcal{X}_{t_1} \times \mathcal{X}_{t_2} \times (\mathbb{R}^{n})^{t_2 - t_1 - 1} \times \left(\mathbb{R}^{m}\right)^{t_2 - t_1}.\]
And since the objective function is strongly convex, the optimal solution set is a singleton. Thus, function $\psi$ is well-defined. By Corollary 3.1 in \cite{lee2006continuity}, we know that $\psi_{t_1}^{t_2}$ is a continuous function in $\upsilon_{t_1}^{t_2}$.

We will consider the path from $\upsilon_{t_1}^{t_2}$ to $(\upsilon_{t_1}^{t_2})'$ given by the line segment
\[\lambda (\upsilon_{t_1}^{t_2})' + (1 - \lambda) \upsilon_{t_1}^{t_2}, \lambda \in [0, 1].\]
We define a mapping $\xi: [0, 1] \to \{0, 1\}^{E}$, that denotes which subset of the $E := \sum_{\tau = t_1 + 1}^{t_2 - 1} \alpha_\tau + \sum_{\tau = t_1}^{t_2 - 1} \beta_\tau$ inequality constraints of optimization problem $\psi_{t_1}^{t_2}$ are active at $\lambda (\upsilon_{t_1}^{t_2})' + (1 - \lambda) \upsilon_{t_1}^{t_2}$. The $E$ constraints are listed in this order:
\begin{align*}
    &\{\left(N_\tau x_{\tau}\right)_i \leq \left(p_\tau\right)_i, \text{ for } i = 1, \ldots, \alpha_\tau\}, \text{ for }\tau = t_1 + 1, \ldots, t_2 - 1,\\
    &\{\left(M_\tau u_{\tau}\right)_i \leq \left(q_\tau\right)_i, \text{ for } i = 1, \ldots, \beta_\tau\}, \text{ for }\tau = t_1, \ldots, t_2 - 1
\end{align*}
For each $(0, 1)$ vector $s \in \{0, 1\}^{E}$ (which denotes the set of active constraints in $\psi_{t_1}^{t_2}$), we define the following auxiliary equality constrained optimization problem:
\begin{subequations}\label{equ:auxiliary_control_problem:equ-constraints}
\begin{align}
    \phi_s\left(\upsilon_{t_1}^{t_2}\right) = \argmin_{x_{t_1:t_2}, u_{t_1:t_2-1}} &\sum_{t = t_1+1}^{t_2-1} f_t(x_t, w_t) + \sum_{t=t_1}^{t_2-1} c_t(u_t, \delta_t)\nonumber\\*
    \text{ s.t. }&x_t = A_{t-1} x_{t-1} + B_{t-1} u_{t-1}, \text{for } t = t_1, \ldots, t_2,\nonumber\\*
    &(N_t x_t)_i = (p_t)_i, \text{if }t \in (t_1, t_2) \text{ and } s_{j} = 1 \text{ for }j = \sum_{\tau = t_1+1}^{t-1}\alpha_\tau + i,\\*
    &u_t \in \mathcal{U}_t \subseteq \mathbb{R}^m, \forall t_1 \leq t < t_2,\nonumber\\*
    &x_{t_1} = y_{t_1}, x_{t_2} = y_{t_2},\nonumber
\end{align}
\end{subequations}
Let $\eta_s(\upsilon_{t_1}^{t_2})$ denote the optimal value of \eqref{equ:auxiliary_control_problem:equ-constraints}. Note that $\phi_s\left(\upsilon_{t_1}^{t_2}\right)$ does not exist for many $s \in \{0, 1\}^{E}$, but this does not affect our analysis. Since the cost functions are quadratic, we know that $\phi_s\left(\upsilon_{t_1}^{t_2}\right)$ is an affine function of $\upsilon_{t_1}^{t_2}$, and $\eta_s(\upsilon_{t_1}^{t_2})$ is a quadratic function of $\upsilon_{t_1}^{t_2}$ if they exists.

\begin{lemma}\label{lemma:switching-cost-opt-aux-original-equivalence}
For any $\lambda \in [0, 1]$, let $s \coloneqq \xi(\lambda)$. Then, we have
\begin{align*}
    \psi_{t_1}^{t_2}\left(\lambda (\upsilon_{t_1}^{t_2})' + (1 - \lambda) \upsilon_{t_1}^{t_2}\right) ={}& \phi_s\left(\lambda (\upsilon_{t_1}^{t_2})' + (1 - \lambda) \upsilon_{t_1}^{t_2}\right),\\
    \iota_{t_1}^{t_2}\left(\lambda (\upsilon_{t_1}^{t_2})' + (1 - \lambda) \upsilon_{t_1}^{t_2}\right) ={}& \eta_s\left(\lambda (\upsilon_{t_1}^{t_2})' + (1 - \lambda) \upsilon_{t_1}^{t_2}\right).
\end{align*}
\end{lemma}
\begin{proof}[Proof of \Cref{lemma:switching-cost-opt-aux-original-equivalence}]
Note that
\[\iota_{t_1}^{t_2}\left(\lambda (\upsilon_{t_1}^{t_2})' + (1 - \lambda) \upsilon_{t_1}^{t_2}\right) \geq \eta_s\left(\lambda (\upsilon_{t_1}^{t_2})' + (1 - \lambda) \upsilon_{t_1}^{t_2}\right)\]
because the optimization problem on the RHS has less constraints. If the inequality holds with equality, we must have
\[\psi_{t_1}^{t_2}\left(\lambda (\upsilon_{t_1}^{t_2})' + (1 - \lambda) \upsilon_{t_1}^{t_2}\right) = \phi_s\left(\lambda (\upsilon_{t_1}^{t_2})' + (1 - \lambda) \upsilon_{t_1}^{t_2}\right)\]
since the optimal solution for the LHS is feasible for the RHS by the assumption on active constraints, and the optimization problem on RHS has a unique solution. Otherwise, we must have
\begin{align*}
    \psi_{t_1}^{t_2}\left(\lambda (\upsilon_{t_1}^{t_2})' + (1 - \lambda) \upsilon_{t_1}^{t_2}\right) \not ={}& \psi_s\left(\lambda (\upsilon_{t_1}^{t_2})' + (1 - \lambda) \upsilon_{t_1}^{t_2}\right),\\
    \iota_{t_1}^{t_2}\left(\lambda (\upsilon_{t_1}^{t_2})' + (1 - \lambda) \upsilon_{t_1}^{t_2}\right) >{}& \eta_s\left(\lambda (\upsilon_{t_1}^{t_2})' + (1 - \lambda) \upsilon_{t_1}^{t_2}\right).
\end{align*}
Consider the convex combination $\zeta(\kappa)$ for $\kappa \in [0, 1]$ defined as
\[\zeta(\kappa) = (1-\kappa) \psi_{t_1}^{t_2}\left(\lambda (\upsilon_{t_1}^{t_2})' + (1 - \lambda) \upsilon_{t_1}^{t_2}\right) + \kappa \phi_s\left(\lambda (\upsilon_{t_1}^{t_2})' + (1 - \lambda) \upsilon_{t_1}^{t_2}\right).\]
Note that $\zeta(\kappa)$ satisfies all constraints in $s$ because they are active for all $\kappa \in [0, 1]$. Since the constraints of $\psi_{t_1}^{t_2}$ that are not in $s$ are inactive at $\eta = 0$, there must exist $\kappa > 0$ such that $\zeta(\kappa)$ is also feasible for $\psi_{t_1}^{t_2}$. $\zeta(\kappa)$ has a strictly smaller cost than $\zeta(0) = \psi_{t_1}^{t_2}\left(\lambda (\upsilon_{t_1}^{t_2})' + (1 - \lambda) \upsilon_{t_1}^{t_2}\right)$, which leads to a contradiction.
\end{proof}

\yiheng{If LICQ is not satisfied, the optimal value function of a quadratic program might not be differentiable. To see this, for $y \in \mathbb{R}^2$, consider
\[g(y) = \min_{x \in \mathbb{R}^2} x^2, \text{ s.t. } x \geq y_1, x \geq y_2.\]
At point $y = (1, 1)$, the directional derivative in direction $(0, 1)$ is $2$, but the directional derivative in direction $(0, -1)$ is $0$.
}

==> problem_setting_old.tex <==
We consider a finite-horizon discrete-time online control problem with linear time-varying (LTV) dynamics, time-varying costs, and constraints, namely
\begin{align}\label{equ:online_control_problem}
    \min_{x_{0:T}, u_{0:T-1}} &\sum_{t = 1}^{T} f_t(x_t, w_t) + \sum_{t=0}^{T-1} c_t(u_t, \delta_t)\nonumber\\*
    \text{ s.t. }&x_t = A_{t-1} x_{t-1} + B_{t-1} u_{t-1}, &\forall 0 < t \leq T,\nonumber\\*
    &x_t \in \mathcal{X}_t \subseteq \mathbb{R}^n, &\forall 0 < t \leq T,\\*
    &u_t \in \mathcal{U}_t \subseteq \mathbb{R}^m, &\forall 0 \leq t < T,\nonumber\\*
    &x_0 = x(0), x_T = x(T),\nonumber
\end{align}
where the costs functions are quadratic and given by
\[f_t(x_t, w_t) \coloneqq (x_t - w_t)^\top Q_t (x_t - w_t),\text{ and } c_t(u_t, \delta_t) \coloneqq (u_t - \delta_t)^\top R_t (u_t - \delta_t).\]
Here matrix $Q_t$ and $R_t$ satisfies that
\[\mu_f I \preceq Q_t \preceq \ell_f I, \text{ and }0 \preceq R_t \preceq \ell_f I.\]
The constraint sets $\mathcal{X}_t$ and $\mathcal{U}_t$ are convex polytopes given by
\[\mathcal{X}_t = \{x \in \mathbb{R}^n \mid N_t x \leq p_t\}, \text{ and } \mathcal{U}_t = \{u \in \mathbb{R}^m \mid M_t u \leq q_t\},\]
where $N_t \in \mathbb{R}^{\alpha_t \times n}$ and $M_t \in \mathbb{R}^{\beta_t \times m}$.

\begin{assumption}\label{assump:controllability}
We assume that for any time $t$, given any $x \in \mathcal{X}_t$, there exists $u \in \mathcal{U}_t$ such that $A_t x + B_t u \in \mathcal{X}_{t+1}$. Further, there exists a positive integer $d$ such that for any time $t$ and $t' \geq t + d$, for arbitrary $x_t \in \mathcal{X}_t$ and $x_{t'} \in \mathcal{X}_{t'}$, there exists a feasible trajectory from $x_t$ to $x_{t'}$:
\[x_t \xrightarrow{u_t} x_{t+1} \xrightarrow{u_{t+1}} \cdots \xrightarrow{u_{t'-1}} x_{t'}.\]
\end{assumption}

To simplify the notation, for time $t_1$ and $t_2$ that satisfies $t_2 \geq t_1 + d$, we define $\psi_{t_1}^{t_2}\left(y_{t_1}, y_{t_2}, w_{t_1+1:t_2-1}, \delta_{t_1:t_2-1}\right)$ as the unique solution to the following auxiliary optimization problem:
\begin{align}\label{equ:auxiliary_control_problem}
    \argmin_{x_{t_1:t_2}, u_{t_1:t_2-1}} &\sum_{t = t_1+1}^{t_2-1} f_t(x_t, w_t) + \sum_{t=t_1}^{t_2-1} c_t(u_t, \delta_t)\nonumber\\*
    \text{ s.t. }&x_t = A_{t-1} x_{t-1} + B_{t-1} u_{t-1}, &\forall t_1 < t \leq t_2,\nonumber\\*
    &x_t \in \mathcal{X}_t \subseteq \mathbb{R}^n, &\forall t_1 < t < t_2,\\*
    &u_t \in \mathcal{U}_t \subseteq \mathbb{R}^m, &\forall t_1 \leq t < t_2,\nonumber\\*
    &x_{t_1} = y_{t_1}, x_{t_2} = y_{t_2},\nonumber
\end{align}
where the parameters $\left(y_{t_1}, y_{t_2}\right) \in \mathcal{X}_{t_1} \times \mathcal{X}_{t_2}$. By Assumption \ref{assump:controllability}, the function $\psi_{t_1}^{t_2}$ is well-defined. Let $\iota_{t_1}^{t_2}\left(y_{t_1}, y_{t_2}, w_{t_1+1:t_2-1}, \delta_{t_1:t_2-1}\right)$ denote the optimal value of the optimization problem \eqref{equ:auxiliary_control_problem}.

\begin{assumption}\label{assump:uniform-controllability}
There exists a universal constant $\sigma > 0$ that satisfies the following property: For any time $t$ and $t' \in [t+d, t+2d)$, if a block matrix
\begin{align}
    D \coloneqq \left[\begin{array}{cccccccc}
        B_t & - I & & & & & & \\
         & A_{t+1} & B_{t+1} & - I & & & & \\
         & & & A_{t+2} & B_{t+2} & - I & & \\
         & & & & & \ddots & & \\
         & & & & & & A_{t'-1} & B_{t'-1}\\
         \hdashline
         \tilde{M}_t & & & & & & & \\
          & \tilde{N}_{t+1} & & & & & & \\
          & & \tilde{M}_{t+1} & & & & & \\
          & & & \tilde{N}_{t+2} & & & & \\
          & & & & \tilde{M}_{t+2} & & & \\
          & & & & & \ddots & & \\
          & & & & & & \tilde{N}_{t'-1} & \\
          & & & & & & & \tilde{M}_{t'-1}
    \end{array}
    \right]
\end{align}
satisfies that each $\tilde{M}_\tau$ is formed by a subset (can be $\emptyset$) of the rows in $M_\tau$, and each $\tilde{N}_\tau$ is formed by a subset (can be $\emptyset$) of the rows in $N_\tau$. If $\sigma_{min}(D) > 0$, then $\sigma_{min}(D) \geq \sigma$.
\end{assumption}

==> soco_perturbation_bounds.tex <==
\begin{theorem}\label{thm:SOCO-sensitivity}
Given a tuple $\left(\hat{y}_0, \hat{y}_\horizonvar, \zeta_{1:H-1}^f, \zeta_{0:H-1}^c\right)$ that contains the initial state, the terminal state, and the parameters for the hitting/switching costs in this order, we consider the optimal solution of the constrained SOCO problem
\begin{align}\label{equ:large-scale-SOCO}
    \hat{\psi}\left(\hat{y}_0, \hat{y}_\horizonvar, \zeta_{1:H-1}^f, \zeta_{0:H-1}^c\right) \coloneqq \argmin_{\hat{x}_{1:\horizonvar-1}}& \sum_{\tau=1}^{\horizonvar-1} \hat{f}_\tau(\hat{x}_\tau, \zeta_\tau^f) + \sum_{\tau=1}^{\horizonvar} \hat{c}_\tau(\hat{x}_\tau, \hat{x}_{\tau - 1}, \zeta_{\tau-1}^c)\nonumber\\*
    \text{ s.t. }& \hat{x}_\tau \in \hat{\mathcal{X}}_\tau \subseteq \mathbb{R}^n, &\forall 0 < \tau < H,\nonumber\\*
    &\hat{x}_0 = \hat{y}_0, \hat{x}_\horizonvar = \hat{y}_\horizonvar,
\end{align}
indexed by $1, \ldots, \horizonvar-1$. Assume the hitting cost $\hat{f}_\tau: \hat{\mathcal{X}}_\tau \times \mathbb{R}^{r_f} \to \mathbb{R}$ is convex and $\hat{\ell}_f$-smooth, and $\hat{f}_\tau\left(\cdot, \zeta_\tau^f\right)$ is $\hat{\mu}_f$-strongly convex for any fixed parameter $\zeta_\tau^f$. The switching cost $\hat{c}_\tau: \hat{\mathcal{X}}_\tau \times \hat{\mathcal{X}}_{\tau-1} \times \mathbb{R}^{r_c} \to \mathbb{R}$ is convex and $\hat{\ell}_c$-smooth. Here $\hat{\mathcal{X}}_\tau$ is a convex subset of $\mathbb{R}^n$ for $\tau = 0, \ldots, H$. Then, for any $\left(\hat{y}_0, \hat{y}_\horizonvar, \zeta_{1:H-1}^f, \zeta_{0:H-1}^c\right), \left(\hat{y}_0', \hat{y}_\horizonvar', (\zeta_{1:H-1}^f)', (\zeta_{0:H-1}^c)'\right) \in \hat{\mathcal{X}}_0 \times \hat{\mathcal{X}}_H \times \mathbb{R}^{H \times r} \times \mathbb{R}^{H \times r}$,
\begin{align*}
    &\norm{\hat{\psi}\left(\hat{y}_0, \hat{y}_\horizonvar, \zeta_{1:H-1}^f, \zeta_{0:H-1}^c\right)_h - \hat{\psi}\left(\hat{y}_0', \hat{y}_\horizonvar', (\zeta_{1:H-1}^f)', (\zeta_{0:H-1}^c)'\right)_h}\\
    \leq{}& C_0\bigg(\decayvar_0^{h}\norm{\hat{y}_0 - \hat{y}_0'} + \sum_{\tau=1}^{\horizonvar-1} \decayvar_0^{\abs{h - \tau}}\norm{\zeta_\tau^f - (\zeta_\tau^f)'} + \sum_{\tau = 0}^{\horizonvar-1}\decayvar_0^{\abs{h - \tau}}\norm{\zeta_\tau^c - (\zeta_\tau^c)'} + \decayvar_0^{\horizonvar-h}\norm{\hat{y}_\horizonvar - \hat{y}_\horizonvar'} \bigg)
\end{align*}
for all $1 \leq h \leq \horizonvar-1$, where
\begin{align*}
    \lambda_0 &= \lambda_0(\hat{\mu}_f, \hat{\ell}_f, \hat{\ell}_c) = \left(1 - \frac{\hat{\mu}_c}{\hat{\ell}_f + 2\hat{\ell}_c}\right)^{\frac{1}{2}},\\
    C_0 &= C_0(\hat{\mu}_f, \hat{\ell}_f, \hat{\ell}_c) = \frac{\hat{\ell}_f + 2\hat{\ell}_c + \sqrt{(\hat{\ell}_f + 2\hat{\ell}_c)^2 + 4(\hat{\ell}_f + 2\hat{\ell}_c + \max(\hat{\ell}_f, \hat{\ell}_c))}}{2\hat{\mu}_f \decayvar_0^{\frac{1}{2}}}.
\end{align*}
\end{theorem}

\yiheng{Compared with existing SOCO perturbation bounds, \Cref{thm:SOCO-sensitivity} are novel in the following ways:
\begin{enumerate}
    \item It does not require the cost functions to have second order derivatives (Most important);
    \item The constraint set $\hat{\mathcal{X}}_\tau$ can be arbitrary convex set. In our ICML submission, it has to be a polytope with non-empty interior;
    \item The parameter in hitting cost function is also considered, so we can study the prediction error on hitting cost functions.
\end{enumerate}
}

A key lemma we need to show \Cref{thm:SOCO-sensitivity} is \Cref{lemma:Lipschitzness-of-global-optimal-solution} about the Lipschitzness of the global optimal solution of \eqref{equ:large-scale-SOCO}.

\begin{lemma}\label{lemma:Lipschitzness-of-global-optimal-solution}
Under the same assumption as \Cref{thm:SOCO-sensitivity}, the optimal solution $\hat{\psi}(\hat{y}_0, \zeta, \hat{y}_\horizonvar)$ is $L_1$-Lipschitz in its parameters, i.e.,
\begin{align*}
    &\norm{\hat{\psi}\left(\hat{y}_0, \hat{y}_\horizonvar, \zeta_{1:H-1}^f, \zeta_{0:H-1}^c\right) - \hat{\psi}\left(\hat{y}_0', \hat{y}_\horizonvar', (\zeta_{1:H-1}^f)', (\zeta_{0:H-1}^c)'\right)}\\
    \leq{}& L_1 \sqrt{\norm{\hat{y}_0 - \hat{y}_0'}^2 + \sum_{\tau = 1}^{\horizonvar - 1} \norm{\zeta_\tau^f - (\zeta_\tau^f)'}^2 + \sum_{\tau = 0}^{\horizonvar - 1} \norm{\zeta_\tau^c - (\zeta_\tau^c)'}^2 + \norm{\hat{y}_\horizonvar - \hat{y}_\horizonvar'}^2},
\end{align*}
where $L_1 = L_1(\hat{\mu}_f, \hat{\ell}_f, \hat{\ell}_c) = \frac{\hat{\ell}_f + 2\hat{\ell}_c + \sqrt{(\hat{\ell}_f + 2\hat{\ell}_c)^2 + 4(\hat{\ell}_f + 2\hat{\ell}_c + \max(\hat{\ell}_f, \hat{\ell}_c))}}{2\hat{\mu}_f}$.
\end{lemma}

\begin{proof}[Proof of \Cref{lemma:Lipschitzness-of-global-optimal-solution}]
\input{Proofs/Lipschitz-global-opt-sol}
\end{proof}

Before showing \Cref{thm:SOCO-sensitivity}, we first recall a result about the convergence rate of gradient descent for a well-conditioned function $\hat{F}$ on a constraint set $\hat{\mathcal{Q}}$.

\begin{theorem}\label{thm:well-cond-grad-descent-with-constraints}
Let $\hat{F}$ be a $\hat{\mu}_F$-strongly convex and $\hat{\ell}_F$-smooth function on $\mathbb{R}^{n_0}$. Assume the constraint set $\hat{\mathcal{Q}} \subseteq \mathbb{R}^{n_0}$ is a closed convex set. Consider the iterative gradient-based update rule
\begin{align}\label{thm:well-cond-grad-descent-with-constraints:update-rule}
    z(s+1) = z(s) - \frac{1}{\hat{\ell}_F} g_{\hat{\mathcal{Q}}}\left(z(s); \hat{\ell}_F\right), \text{ for }s = 0, 1, \ldots, \text{ with } z(0) \in \hat{\mathcal{Q}},
\end{align}
where $g_{\hat{\mathcal{Q}}}\left(z(s); \hat{\ell}_F\right)$ denotes the gradient mapping of $\hat{F}$ on $\hat{\mathcal{Q}}$, which is defined as
\begin{subequations}\label{thm:well-cond-grad-descent-with-constraints:gradient-map}
\begin{align}
    z_{\hat{\mathcal{Q}}}\left(\bar{z}; \gamma\right) ={}& \argmin_{z \in \hat{\mathcal{Q}}}\left(\hat{F}(\bar{z}) + \langle \nabla\hat{F}(\bar{z}), z - \bar{z}\rangle + \frac{\gamma}{2}\norm{z - \bar{z}}^2\right),\label{thm:well-cond-grad-descent-with-constraints:gradient-map:s1}\\
    g_{\hat{\mathcal{Q}}}(\bar{z}; \gamma) ={}& \gamma\left(\bar{z} - z_{\hat{\mathcal{Q}}}(\bar{z}; \gamma)\right)\label{thm:well-cond-grad-descent-with-constraints:gradient-map:s2}
\end{align}
for any fixed $\gamma > 0$. Define $z^* \coloneqq \argmin_{z \in \hat{\mathcal{Q}}}\hat{F}(z)$. Then, we have that
\[\norm{z(s) - z^*}^2 \leq \left(1 - \frac{\hat{\mu}_F}{\hat{\ell}_F}\right)^s \norm{z(0) - z^*}^2.\]
\end{subequations}
\end{theorem}

Now we come back to the proof of \Cref{thm:SOCO-sensitivity}.

\begin{proof}[Proof of \Cref{thm:SOCO-sensitivity}]
\input{Proofs/SOCO-sensitivity}
\end{proof}
